Safe Learning-Based Control of Stochastic Jump Linear Systems: a Distributionally Robust Approach

We consider the problem of designing control laws for stochastic jump linear systems where the disturbances are drawn randomly from a finite sample space according to an unknown distribution, which is estimated from a finite sample of i.i.d. observations. We adopt a distributionally robust approach to compute a mean-square stabilizing feedback gain with a given probability. The larger the sample size, the less conservative the controller, yet our methodology gives stability guarantees with high probability, for any number of samples. Using tools from statistical learning theory, we estimate confidence regions for the unknown probability distributions (ambiguity sets) which have the shape of total variation balls centered around the empirical distribution. We use these confidence regions in the design of appropriate distributionally robust controllers and show that the associated stability conditions can be cast as a tractable linear matrix inequality (LMI) by using conjugate duality. The resulting design procedure scales gracefully with the size of the probability space and the system dimensions. Through a numerical example, we illustrate the superior sample complexity of the proposed methodology over the stochastic approach.

==> Stability.tex <==
%!TEX root=./main.tex 
\section{Distributional stability margin} \label{sec:stability-margin}


==> Tractable.tex <==
%!TEX root = ./main.tex

\section{Tractable reformulations}

Solving \eqref{eq:robust-lyapunov} is generally not straightforward. 
A simple way of avoiding the maximization over all distributions in the ambiguity set is to exploit the structure of the used distance metric. 
If the norm balls corresponding to the used distance metric are polytopes, a possible approach is to construct the (finite, discrete) set
\(\mathcal{V}(\hat{p}) =
\lbrace{p \in \Df \vert \dist(p, \hat{p})=\epsilon\rbrace}\)
of vertices of the intersection between the distance polytope with the probability simplex and impose \eqref{eq:linear-lyapunov} for all
\(p \in \mathcal{V}(\hat{p})\). \remark{Missing proof/citation for this}

This means that for an ambiguity set with \(n_v\) vertices, \(n_v\) problems of the form \eqref{eq:linear-lyapunov} need to be solved. For discrete distributions, \eqref{eq:linear-lyapunov} reduces to 
\begin{equation} \label{eq:discrete-linear-lyapunov}
	\sum_{\omega \in \Omega} p_{\omega} \big[ A(\omega) + B(\omega)K \big]^T P \big[ A(\omega) + B(\omega)K \big] - P \leq -Q. 
\end{equation}
One can easily show that this problem can be transformed into a linear matrix inequality (LMI). For ease of notation, consider the expression  
\[ 
	\sum_{i=1}^n p_i D_i^T M D_i - M.
\]
We now define
\(\tilde{D} = \big[\sqrt{p_1} D_1^T, \ldots, \sqrt{p_n} D_n^T \big]^T\) and \(\tilde{M} = I_n \otimes M \), \remark{add to notation section} so that 
\[ 
	\sum_{i=1}^n p_i D_i^T M D_i = \tilde{D}^T \tilde{M} \tilde{D}.
\]

Similarly, for \eqref{eq:discrete-linear-lyapunov}, we can define \(\tilde{A}\), \(\tilde{B}\) and \(\tilde{P}\), so that \eqref{eq:discrete-linear-lyapunov} is equivalent to
\[ 
[\tilde{A} + \tilde{B}K]^T \tilde{P}[\tilde{A} + \tilde{B}K] - P \leq -Q. 
\]
Since both \(P\) and \(K\) are unknown variables, this condition forms a bilinear matrix inequality (BMI). However, using a standard procedure based on the Schur complement\footnote{\remark{\url{http://staff.uz.zgora.pl/wpaszke/materialy/ts/LMISlides1.pdf}, find proper reference to cite}}, this BMI can be shown to be equivalent to the following LMI 
\[
\left[
	\begin{matrix}
	 -\tilde{W} & \tilde{A} W + \tilde{B} N \\ 
	 W \tilde{A}^T + N^T \tilde{B}^T & - W
	\end{matrix} 
\right] \leq 0
\]
where \(W \dfn P^{-1} \), \( \tilde{W} = \tilde{P}^{-1} = I_n \otimes W^{-1}\) and \(N \dfn K W\). 


\subsection{Total variation distance}

The total variation (\TV) distance for discrete distributions \(p, q \in \Df_n\) \remark{(Define \(\Df_n\) under ``notation''-subsection to denote the \(n\)-dimensional probability simplex} is defined as
\[
	\dist_{\mathrm{TV}}(p, q) = \frac{1}{2} \sum_{i=1}^{n} \lvert p_i - q_i \rvert.
\]
The vertices of the ambiguity set \(\Af_{\epsilon}(\hat{p}) \dfn 
\{p\in\Df_n {}\mid{} \dist_{\mathrm{TV}}(p, \hat{p}) \leq \epsilon\}\) are the vertices of 
\[
	\mathcal{B}_{\epsilon}^{\mathrm{TV}}(\hat{p}) \cap \Df_n
\]
\textcolor{gray}{Later we use the total variation distance without the ``\(\tfrac{1}{2}\)''}
